ReDraft, Don't Just Distill: Reference-Driven Revision for Continual VLLM Post-Training

Continual post-training of large multimodal models should add new capabilities while preserving those from pre-training, and the two goals pull in opposite directions. SFT gives explicit target supervision that learns a task from near-zero accuracy, but its off-policy targets move the model far enough to cause forgetting; on-policy methods such as RLVR and self-distillation preserve policy proximity yet supply little signal when the policy cannot yet solve the task. We introduce ReDraft (Reference-Driven Revision and Fine-Tuning), which obtains both from the model's own failures: using an expert response only as a reference, it has the model revise its own incorrect rollout, keeps the revision only if a verifier accepts it, and fine-tunes on what survives. Each retained target is therefore explicit, yet still close to the current policy. Across Counting, Clock Reading, and Jigsaw on Qwen2.5-VL-3B/7B, two of them with near-zero accuracy, ReDraft gains 56.9 points on the target task against SFT's 52.9 while cutting prior-task loss from 16.6 to 1.5 points (11.3x less forgetting), and improves on OPSD along both axes (19.3 gain, 6.2 loss). Data- and parameter-space analyses match the design: revised targets are more probable under the base model, and the updates they induce stay compact and follow SFT's direction more closely than OPSD's. Together, these results show that revising the model's own rollout rather than directly imitating an expert trajectory can reconcile cold-start acquisition with prior-capability retention.

==> appendices/demo_box_styles.tex <==
% Shared rounded-box styles for qualitative demos.
% Requires: \usepackage[most]{tcolorbox}, float, placeins.

\makeatletter
\ifdefined\XeTeXrevision
  \@ifpackageloaded{fontspec}{}{\usepackage{fontspec}}
  \IfFontExistsTF{Latin Modern Mono}{%
    \newfontfamily\DemoMono{Latin Modern Mono}[Scale=MatchLowercase]%
  }{%
    \IfFontExistsTF{Menlo}{%
      \newfontfamily\DemoMono{Menlo}[Scale=MatchLowercase]%
    }{%
      \newcommand{\DemoMono}{\ttfamily}%
    }%
  }%
\else
  \ifdefined\luatexversion
    \@ifpackageloaded{fontspec}{}{\usepackage{fontspec}}
    \IfFontExistsTF{Latin Modern Mono}{%
      \newfontfamily\DemoMono{Latin Modern Mono}[Scale=MatchLowercase]%
    }{%
      \newcommand{\DemoMono}{\ttfamily}%
    }%
  \else
    \newcommand{\DemoMono}{\ttfamily}%
  \fi
\fi
\makeatother

\definecolor{DemoInputFrame}{HTML}{667085}
\definecolor{DemoInputTitle}{HTML}{475467}
\definecolor{DemoInputBack}{HTML}{F8FAFC}
\definecolor{DemoExampleFrame}{HTML}{4B5563}
\definecolor{DemoExampleTitle}{HTML}{374151}
\definecolor{DemoExampleBack}{HTML}{FFFFFF}
\definecolor{DemoWrongFrame}{HTML}{B95A45}
\definecolor{DemoWrongTitle}{HTML}{8E3B2A}
\definecolor{DemoWrongBack}{HTML}{FBF3F0}
\definecolor{DemoRightFrame}{HTML}{4A8F73}
\definecolor{DemoRightTitle}{HTML}{2F6B54}
\definecolor{DemoRightBack}{HTML}{F1F7F3}
\definecolor{DemoTemplateFrame}{HTML}{A07A33}
\definecolor{DemoTemplateTitle}{HTML}{7A5A1E}
\definecolor{DemoTemplateBack}{HTML}{FAF6EC}


\tcbset{
  demobase/.style={
    enhanced,
    breakable,
    boxrule=0.8pt,
    arc=2mm,
    left=7pt,
    right=7pt,
    top=6pt,
    bottom=6pt,
    toptitle=3pt,
    bottomtitle=3pt,
    lefttitle=7pt,
    righttitle=7pt,
    before skip=8pt,
    after skip=8pt,
    fontupper={\footnotesize\DemoMono\raggedright},
    fonttitle=\bfseries\small,
    coltitle=white,
  },
  demoinput/.style={
    demobase,
    unbreakable,
    fontupper={\normalfont},
    colback=DemoInputBack,
    colframe=DemoInputFrame,
    colbacktitle=DemoInputTitle,
    title={#1},
  },
  demoexample/.style={
    demobase,
    fontupper={\small\raggedright},
    colback=DemoExampleBack,
    colframe=DemoExampleFrame,
    colbacktitle=DemoExampleTitle,
    title={#1},
  },
  demowrong/.style={
    demobase,
    colback=DemoWrongBack,
    colframe=DemoWrongFrame,
    colbacktitle=DemoWrongTitle,
    title={Incorrect Rollout},
  },
  demoright/.style={
    demobase,
    colback=DemoRightBack,
    colframe=DemoRightFrame,
    colbacktitle=DemoRightTitle,
    title={Revised Response},
  },
  demotemplate/.style={
    demobase,
    colback=DemoTemplateBack,
    colframe=DemoTemplateFrame,
    colbacktitle=DemoTemplateTitle,
    title={#1},
  },
}

